Input-to-State Stability in Probability

Input-to-State Stability (ISS) is fundamental in mathematically quantifying how stability degrades in the presence of bounded disturbances. If a system is ISS, its trajectories will remain bounded, and will converge to a neighborhood of an equilibrium of the undisturbed system. This graceful degradation of stability in the presence of disturbances describes a variety of real-world control implementations. Despite its utility, this property requires the disturbance to be bounded and provides invariance and stability guarantees only with respect to this worst-case bound. In this work, we introduce the concept of ``ISS in probability (ISSp)'' which generalizes ISS to discrete-time systems subject to unbounded stochastic disturbances. Using tools from martingale theory, we provide Lyapunov conditions for a system to be exponentially ISSp, and connect ISSp to stochastic stability conditions found in literature. We exemplify the utility of this method through its application to a bipedal robot confronted with step heights sampled from a truncated Gaussian distribution.

==> oldproof_lyap2ISSp.tex <==
\begin{proof}
We begin by constructing a nonnegative supermartingale $W(\mb{x}_k, k)$ via a time-varying, affine transform of the Lyapunov function $V(\mb{x}_k)$. Rearranging the Lyapunov drift condition \eqref{eq:delta_v} with $\kappa_3(r) = \alpha r$ for some $\alpha \in (0,1) $ , we can see that $V(\mb{x}_k)$ almost resembles a supermartingale\footnote{Note that $\E{V(\mb{x}_{k+1}) \mid \mb{x}_k} = \E{V(\mb{x}_{k+1}) \mid \mb{x}_{0:k}}$ since system \eqref{eq:dt_dynamics} is Markovian.},
\begin{align}
    \E{V(\mb{x}_{k+1}) \mid \mb{x}_k} \leq (1 - \alpha) V(\mb{x}_k) + \delta \Vert \mb{d} \Vert_p^c,
\end{align}
but with a scaling $(1-\alpha)$ and additive constant $\delta \Vert \mb{d} \Vert_p^c$. 

Thus, for a particular horizon $K\in \mathbb{N}$, we construct $W(\mb{x}_k, k)$ by undoing this scaling and translation. Letting $W_k \triangleq W(\mb{x}_k, k)$ for notational simplicity, this construction is:
% \begin{align}
%     W(\mb{x}_k) = \theta^k V(\mb{x}_k) + \delta \Vert \mb{d} \Vert_p^c \left(\sum_{i=1}^K \theta^i - \sum_{i=1}^k \theta^{i} \right),
% \end{align}
\begin{align}
    W_k = \underbrace{\theta^k V(\mb{x}_k)}_{\textrm{rescale}} - \underbrace{\delta \Vert \mb{d} \Vert_p^c \sum_{i=1}^k \theta^{i}}_{\textrm{translate}} + \underbrace{\delta \Vert \mb{d} \Vert_p^c \sum_{i=1}^K \theta^i}_{\textrm{ensure } W_k \geq 0 } , 
\end{align}
with $\theta \triangleq \frac{1}{1-\alpha}$ and the constant term $\delta \Vert \mb{d} \Vert_p^c \sum_{i=1}^K \theta^{i}$ added to ensure $W_k \geq 0$.

Next we now show $W_k$ is a nonnegative supermartingale.
We have $W_k \geq 0$ for any $\mb{x}_k \in \mathcal{X},$ since $V(\mb{x}_k) \geq 0$ by definition, and $\theta, \delta, \Vert \mb{d} \Vert_p^c \geq 0.$ Further, we have
\begin{align}
\mathbb{E}\big[&W_{k+1} \mid \mb{x}_k\big] = \mathbb{E} \left[\theta^{k+1} V(\mb{x}_{k+1}) + \delta \Vert \mb{d} \Vert_p^c \sum_{i=k+2}^K \theta^i \right]\\
&\leq \theta^{k+1}\left((1-\alpha) V(\mb{x}_k) + \delta \Vert \mb{d} \Vert_p^c\right) + \delta \Vert \mb{d} \Vert_p^c \sum_{i=k+2}^K \theta^i\label{eq:mart_drift}\\
&= \theta^k V(\mb{x}_k) + \delta \Vert \mb{d} \Vert_p^c \sum_{i=k+1}^K \theta^i = W(\mb{x}_k),\label{eq:mart_simp}
\end{align}
where the inequality \eqref{eq:mart_drift} follows from the drift condition \eqref{eq:delta_v} and \eqref{eq:mart_simp} uses the fact that $\theta = \frac{1}{1-\alpha}.$

Since $W_k$ is a nonnegative supermartingale, we can apply Ville's inequality \eqref{eq:ville} to bound the probability $W_k$ that remains below any $\lambda > 0$ for all $k \leq K$.  Specifically, 
\begin{align}
    \mathbb{P}\Big\{ W(\mb{x}_k) \leq \lambda, \; \forall k \in \{1, \ldots, K \}\Big\} \geq 1 - \frac{W(\mb{x}_0)}{\lambda}.
\end{align}
We also note that, using the geometric series identity $\sum_{i=1}^k \theta^{i-1} = \frac{\theta^k-1}{\theta -1}$, we can write $W_k$ as
\begin{align}
    W_k = \theta^k V(\mb{x}_k) + \frac{\theta \delta \Vert \mb{d} \Vert_p^c (\theta^K - \theta^k)}{\theta - 1} \label{eq:w_geom}
\end{align}

Examining the structure of $W_k,$ if for all $k \in \{1, \ldots, K \}$ we have $W_k \leq \lambda,$ rearranging \eqref{eq:w_geom} results in
\begin{align}
    V(\mb{x}_k) &\leq \left(\lambda - \frac{\theta^{K+1} \delta \Vert \mb{d} \Vert_p^c}{\theta - 1}\right) \theta^{-k} + \delta \Vert \mb{d} \Vert_p^c\\
    &\triangleq M \norm{\mb{x}_0}^c(1 - \alpha)^k + (\delta + \dtwo) \Vert \mb{d} \Vert_p^c
\end{align}
where we define $M \geq 0 $ using the equality $\lambda = M \norm{\mb{x}_0}^c + \frac{\delta \Vert \mb{d} \Vert_p^c}{\alpha(1-\alpha)^{K+1}} + \dtwo \mathcal{D}(\mb{d})^c$ for some $\dtwo \geq 0$ .

Further, using the lower bound \eqref{eq:v_bounds} on $V$, we can write
\begin{align}
    a \norm{\mb{x}_k}^c \leq M \norm{\mb{x}_0}^c (1-\alpha)^k + (\delta + \dtwo) \Vert \mb{d} \Vert_p^c,
\end{align}
for some $a >0$ which, rearranging, and raising both sides to the power of $\frac{1}{c}$ (which preserves order since $c >0$), yields
\begin{align}
    \norm{\mb{x}_k} &\leq \left(\frac{M}{a} \norm{\mb{x}_0}^c (1-\alpha)^k + \frac{(\delta + \dtwo)}{a} \Vert \mb{d} \Vert_p^c\right)^{\frac{1}{c}}\\
    &\leq \left(\frac{M}{a}\right)^\frac{1}{c} \beta \norm{\mb{x}_0} (1 - \alpha)^{\frac{k}{c}} + \beta \left(\frac{(\delta + \dtwo)}{a}\right)^{\frac{1}{c}} \Vert \mb{d} \Vert_p \label{eq:power_split}\\
    &\triangleq \tilde{M} \tilde{\alpha}^k \norm{\mb{x}_0} + \tilde{\delta} \Vert \mb{d} \Vert_p,
\end{align}
for $\tilde{M}, \tilde{\delta} > 0$, $\tilde{\alpha} \in (0, 1) $ and some $\beta>0$ as needed, where the existence of some $\beta$ in \eqref{eq:power_split} follows from Lemma \ref{lemma:power_split} shown in the Appendix. 

Thus, we now must ensure there exists a suitable choice of $M$ such that the probability that this bound holds for all $k \in \{ 1, \ldots, K \}$ is greater than $1-\epsilon.$ By Ville's inequality, 
\begin{align}
    \mathbb{P}&\left\{\norm{\mb{x}_k} \leq \tilde{M} \tilde{\alpha}^k \norm{\mb{x}_0} + \tilde{\delta} \Vert \mb{d} \Vert_p, \; \forall k \in \left\{ 1, \ldots, K \right\} \right\} \nonumber \\ & \geq 1 - \frac{W_0}{\lambda} \\
    &= 1 - \frac{V(\mb{x}_0) + \frac{\theta \delta \Vert \mb{d} \Vert_p^c (\theta^K - 1)}{\theta - 1} }{M \norm{\mb{x}_0}^c + \frac{\theta^{K+1}\delta \Vert \mb{d} \Vert_p^c}{\theta - 1} + \dtwo\mathcal{D}(\mb{d})^c}.
\end{align}
Since this expression is increasing in $M$ and $\dtwo$, as long as $\Vert \mb{x}_0\Vert \neq 0 $ and $ \mathcal{D}(\mb{d}) \neq 0$ we can thus choose $M$ and $\dtwo$ large enough such that 
\begin{align*}
    1 - \frac{V(\mb{x}_0) + \frac{\theta \delta \Vert \mb{d} \Vert_p^c (\theta^K - 1)}{\theta - 1} }{M \norm{\mb{x}_0}^c + \frac{\theta^{K+1}\delta \Vert \mb{d} \Vert_p^c}{\theta - 1} + \dtwo\mathcal{D}(\mb{d})^c} \geq 1 - \epsilon.
\end{align*}
\pc{This is a dodge because I don't want to work out the particular choice of $M$.} 
Thus, for a suitably large $M>0,$ we have $\tilde{M} > 0$, $\tilde{\alpha} \in (0, 1)$ and $\tilde{\delta} > 0$ such that
\begin{align*}
    \mathbb{P}\left\{ \norm{\mb{x}_k} \leq  \tilde{M} \tilde{\alpha}^k \norm{\mb{x}_0} + \tilde{\delta} \Vert \mb{d} \Vert_p, \; k \in \{1, \ldots, K \} \right\} \geq 1 - \epsilon.
\end{align*}
Thus, the system must be E-ISSp, as needed.

\end{proof}

\clearpage
